Solving Epistemic Logic Programs using Generate-and-Test with Propagation

This paper introduces a general framework for generate-and-test-based solvers for epistemic logic programs that can be instantiated with different generator and tester programs, and we prove sufficient conditions on those programs for the correctness of the solvers built using this framework. It also introduces a new generator program that incorporates the propagation of epistemic consequences and shows that this can exponentially reduce the number of candidates that need to be tested while only incurring a linear overhead. We implement a new solver based on these theoretical findings and experimentally show that it outperforms existing solvers by achieving a ~3.3x speed-up and solving 91% more instances on well-known benchmarks.

==> approach-proofs.tex <==
%!TeX root = paper-aaai25.tex
\section{Normal Form}\label{sec:normal.form}

To develop algorithms for solving epistemic logic programs, it is interesting to have a normal form that simplifies the number of cases the algorithm must consider.
%
This also significantly simplifies the presentation of the formal results.
%
We say that an epistemic program is in \emph{normal form} if (i) every subjective literal is of the form~$\K a$ with~$a$ an atom; 
(ii) there are no occurrences of double negated literals;
and (iii) every atom in the program occurs in the head of some rule.
%
We can transform any epistemic program~$\Pi$ into a corresponding program in normal form by 
\begin{itemize}
    \item replacing every literal of the form~$\neg\neg L$ by~$\neg\nott{L}$ and adding rule~$\nott{L} \leftarrow \neg L$ to~$\Pi$;
    
    \item replacing every subjective literal~$\K \neg a$ by~$\K \nott{a}$ and adding rule~$\nott{a} \leftarrow \neg a$ to~$\Pi$;
    \item removing all rules whose body contains a positive%
    %
    \footnote{An occurrence is said to be 
    \emph{negative} if it occurs in the scope of an odd number of negations; it is said to be \emph{positive} otherwise.}
    %
    occurrence of an atom~$a$ that does not occur in the head of any rule; and
    \item removing from the body of all remaining rules all literals that contain a negative occurrence of an atom~$a$ that does not occur in the head of any rule.
\end{itemize}
We assume that for every atom~$a$ in~$\Pi$, atom~$\nott{a}$ do not occur in~$\Pi$.
%
Similarly, we assume that for every literal~$L$ in~$\Pi$, atom~$\nott{L}$ do not occur in~$\Pi$.
%
By~$\NF{\Pi}$ we denote the program obtained from~$\Pi$ by applying the above transformation.
%
In the following result~$\restr{\wv'\!}{\At{\Pi}}$ stands for the set of interpretations obtained from~$\wv'$ by removing all atoms that do not occur in~$\Pi$ from all the interpretations in~$\wv'$.



\begin{theorem}
    Let~$\Pi$ be a program.
    %
    Then, there is a one\nobreakdash-to\nobreakdash-one correspondence between the worldviews of~$\Pi$ and~$\NF{\Pi}$ such that~$\wv$ is a worldview of~$\Pi$ if and only if~$\wv'$ is a worldview of~$\NF{\Pi}$ and~$\wv = \restr{\wv'\!}{\At{\Pi}}$.
\end{theorem}


% This allows us to focus only on programs in normal form, simplifying both the presentation of results as well as the implementation.
% %
% In the rest of the paper, we may present examples that are not in normal form, but we assume that their normal form is computed before applying any algorithm.




\section{Guess-and-Check computation of worldviews}\label{sec:guess-and-check}

% [Son et al., 2017] introduced a guess\nobreakdash-and\nobreakdash-check approach to compute the worldviews of a program under the K15 semantics.??
% %
% [Cabalar et al., ] adapted this approach to compute the worldviews under the G94 semantics.
%
As mentioned in the introduction generate\nobreakdash-and\nobreakdash-test based solvers rely on using two objective programs: a generator program that provides \emph{candidates} and a tester program that checks whether a candidate is a worldview.
%
Algorithm~\ref{alg:guess-and-check} sumarises how to compute~$n$ worldviews using this approach, where~$G(\Pi)$ and~$T(\Pi)$ respectively are a \emph{generator} and a \emph{tester program} for~$\Pi$.
\begin{algorithm}
    \caption{Generate-and-test computation of~$n$ worldviews}\label{alg:guess-and-check}
    \hspace*{\algorithmicindent} \textbf{Input} Generate program $G(\Pi)$\\
    \hspace*{\algorithmicindent} \textbf{Input} Test program $T(\Pi)$\\
    \hspace*{\algorithmicindent} \textbf{Input} Number of requested worldviews~$n$\\
    \hspace*{\algorithmicindent} \textbf{Output} Set~$\Omega$ containing~$n$  worldviews of~$\Pi$

    \begin{algorithmic}[1] %[1] enables line numbers
        \STATE Let $\Omega=\emptyset$.
        \FOR{$M$ in $\SM{G(\Pi)}$}
            \IF {\texttt{Test($T(\Pi)$,$M$)}}
            \STATE $\wv$ = \texttt{BuildWorldView($M$)}
            \STATE $\Omega$ = $\Omega \cup \{ \wv \}$
                \IF {$|\Omega| \geq n$}
                \STATE \textbf{return} $\Omega$
                \ENDIF
            \ENDIF
        \ENDFOR
        \STATE \textbf{return} $\Omega$
    \end{algorithmic}
    % \KwData{Program~$\Pi$, Maximum number of worldviews~$n$}
    % \SetKwFunction{WorldViews}{WorldViews}
    % \SetKwFunction{ExtractAssumptionsAndQueires}{ExtractAssumptionsAndQueires}
    % \SetKwFunction{BuildWorldView}{BuildWorldView}
    % \SetKwFunction{Add}{Add}
    % \SetKwFunction{Test}{Test}
    % \KwResult{Bool}
    %  \WorldViews{$\Pi$, n}\;
    %  \Begin{
    %     $\Omega$ = $\emptyset$\;
    %     \For{{$M$} \textbf{in} {$\SM{G(\Pi)}$}}
    %     {
    %         \label{alg.generator.loop.ini}
    %         % $A,Q$ = \ExtractAssumptionsAndQueires{$M$}\;
    %         % \If{$Q \subseteq \SM{T(\Pi); A}$}
    %         \If{\Test{$T(\Pi)$, $M$}}
    %         {
    %             $\wv$ = \BuildWorldView{$M$}\;
    %             add $\wv$ to $\Omega$\;
    %             \If{$|\Omega| \geq n$}
    %             {
    %                 \Return $\Omega$\;
    %             }
    %         }
    %     }\label{alg.generator.loop.end}
    %     \Return $\Omega$\;
    % }
\end{algorithm}
Different generator and tester programs can be used to compute the worldviews of a program.
%
Here we provide general definitions for these programs with sufficient conditions to ensure that Algorithm~\ref{alg:guess-and-check} correctly computes the worldviews of a program.


We assume that for each subjective literal~$\K a$ in~$\Pi$, there is a new fresh objective atom~$\kk{a}$ that does not occur anywhere else in the program.
%
For simplicity, we assume that no atom occurring in the program starts with the letter~$k$ and, thus, all atoms that start with this letter are newly introduced atoms.
%
We denote by~$K(\Pi)$ the set of these new introduced atoms.
%
Given an interpretation atoms~${M \subseteq \At{\Pi} \cup K(\Pi)}$, we definde~${k(M) = M \cap K(\Pi)}$ as the set of atoms of the form~${\kk{a} \in K(\Pi)}$ that belong to~$M$ with~${a \in \At{\Pi}}$.
%
For a worldview~$\wv$, by~$k(\wv)$ we denote the set of atoms of~$\kk{a} \in K(\Pi)$ such that~$W \models \K a$.
%
Intuitively, each worldview~$\wv$ of~$\Pi$ is associated with a stable model~$M$ of an objective program such that~$k(\wv) = k(M)$.
%
Using this terminology, we can define our general notions of generator and tester program as follows.
%
For an interpretations, by~$\restr{M}{S} = M \cap S$ we denote the set of atoms of~$M$ that belong to~$S$.
%
For a set on interpretations~$\wv$, by~$\restr{\wv}{S}$ we denote the set of interpretations obtained from~$\wv$ by removing all atoms that do not occur in~$S$ from all the interpretations in~$\wv$.



\begin{definition}[Generator Programs]\label{def:generator.program}
We say that an objective program~$G(\Pi)$ is a \emph{generator program} for a program~$\Pi$ if it safisfies the following conditions:
\begin{itemize}
    \item for every worldview~$\wv$ of~$\Pi$, there is a stable model~$M$ of~$G(\Pi)$ satisfying~$k(\wv) = k(M)$ and~$\restr{M}{\At{\Pi}} \in \wv$.
    \item for every stable model~$M$ of~$G(\Pi)$ and every set of interpretations~$\wv$ such that~$k(\wv) = k(M)$, it holds that~$\restr{M}{\At{\Pi}} \in \SM{\Pi^\wv}$.
\end{itemize}
\end{definition}
\noindent
The first condition in Definition~\ref{def:generator.program} ensures that, for every worldview of the original program, the generator program has a stable model that represents that worldview.
%
The second condition ensure that in fact such stable model corresponds to a non\nobreakdash-empty set of interpretations.
%
Recall, that empty sets of interpretations cannot be worldviews.


Before providing our general notion of tester program, let us introduce an example of a tester program.
%
The intuitively idea of a tester program is that it behaves as the subjective reduct of the original program modulo the auxiliary atoms when used in combination with the proper assumptions.
%
For any rule~$r$ of the form of~\eqref{eq:rule}, by~$k(r)$ we denote the result of replacing each subjective literal~$\K a$ by~$\kk{a}$.
%
For any program~$\Pi$, by~$k(\Pi)$ we denote the program obtained from~$\Pi$ by replacing each rule~$r$ of~$\Pi$ by~$k(r)$.
%
Clearly, $k(\Pi)$ is an objective program over~$\At{\Pi} \cup K(\Pi)$.
%
By~$T_0(\Pi)$ we denote the program obtained from~$k(\Pi)$ by adding a choice rule~$\{ \kk{a} \}$ for each atom~$\kk{a} \in K(\Pi)$.
%
The following result shows that~$T_0(\Pi)$ behaves as the subjective reduct of~$\Pi$ modulo the auxiliary atoms under the proper assumptions.


\begin{proposition}\label{prop:basic.tester.program}
    Let~$\Pi$ be a program and~$\wv$ be a set of interpretations.
    %
    Then, 
    \begin{gather}
        \{ M \cup k(\wv) \mid M \in \SM{\Pi^\wv} \} \ = \ \SM{T_0(\Pi); k(\wv)}
        \label{eq:1:prop:basic.generator.tester.program}
    \end{gather}
\end{proposition}

\begin{proof}
    Let~$\mathit{Choices(\Pi)}$ be the program containing choice rule~$\{ \kk{a} \}$ for each atom~$\kk{a} \in K(\Pi)$ and let $\Pi_0$ be the objective program
    \begin{gather*}
        k(\Pi) \cup \mathit{Choices(\Pi)} \cup \{ \neg\neg a \mid a \in k(\wv) \} \cup \{ \neg a  \mid \neg a \in k(\wv) \}.
    \end{gather*}
    By definition, it follows that $\SM{T_0(\Pi); k(\wv)} = \SM{\Pi_0}$.
    %
    Furthermore, program~$\Pi_0$ has the same stable models as program~$\Pi_1 =\Pi_2 \cup \mathit{Facts(\Pi,\wv)}$ where~$\mathit{Facts(\Pi,\wv)} = K(\Pi) \cap k(\wv)$ is the a set of facts for the auxiliary atoms that corresponden to true epistemic atoms in~$\wv$ and~$\Pi_2$ is obtained from~$k(\Pi)$ by removing all rules with an atom~$\kk{a}$ with~$\kk{a} \in \At{\Pi} \setminus k(\wv)$ in the body.
    %
    Note that these atoms cannot be true in~$\Pi_0$ because it contains constraints~$\{ \neg a  \mid \neg a \in k(\wv) \}$ nor in~$\Pi_1$ because they do not occur in the head of any of its rules.
    %
    Moreover, let~$\Pi_3$ be the result of removing all atoms of the form~$\kk{a}$ from~$\Pi_2$.
    %\
    Then~$\Pi_3 = \Pi^\wv$ and~$\SM{\Pi_1} =  \{ M \cup k(\wv) \mid M \in \SM{\Pi_3} \}$.
    %
    Hence, \eqref{eq:1:prop:basic.generator.tester.program} holds.
\end{proof}

\begin{corollary}\label{cor:basic.tester.program}
    Let~$\Pi$ be a program and~$\wv$ be a set of interpretations.
    %
    Then, 
    \begin{gather}
        \SM{\Pi^\wv} \ = \ \restr{\SM{T_0(\Pi); k(\wv)}}{\At{\Pi}}
        \label{eq:1:cor:basic.generator.tester.program}
    \end{gather}
\end{corollary}

The following definition generalizes the above example of tester program.

\begin{definition}[Tester Program]\label{def:tester.program}
We say that an objective program~$T(\Pi)$ is a \emph{tester program} for a program~$\Pi$ if it safisfies the following condition:
\begin{itemize}
    \item every worldview~$\wv$ of~$\Pi$ satisfies~$\wv = \restr{\SM{T(\Pi); k(\wv)}}{\At{\Pi}}$, and
    \item every non\nobreakdash-empty set of interpretations~$\wv$ that is not a worldview of~$\Pi$ satisfies~$\wv \neq \restr{\SM{T(\Pi); k(\wv)}}{\At{\Pi}}$
    % there is a stable model~$M$ of~$G(\Pi)$ satisfying~$k(\wv) = k(M)$ and~$\restr{M}{\At{\Pi}} \in W$.
    % \item for epistemic interpretations~$M \subseteq \At{\Pi} \cup K$, if~$\SM{T(\Pi); k(M)}$ is non\nobreakdash-empty, then it is a worldview of~$\Pi$.
\end{itemize}
\end{definition}


Using Corollary~\ref{cor:basic.tester.program}, it is easy to see that program~$T_0(\Pi)$ is a tester program for~$\Pi$ because any non\nobreakdash-empty set of interpretations~$\wv$ is a worldview iff
\begin{gather*}
    \wv \ = \ \SM{\Pi^\wv} \ =\  \restr{\SM{T(\Pi); k(\wv)}}{\At{\Pi}}
\end{gather*}
Definition~\ref{def:tester.program} does only require that behaves as the subjective reduct on actual worldviews.
%
For non\nobreakdash-worldviews, we only require that it does not produce false positives.
%
This relaxation allow us to introduce further optimizations in the tester program.





\begin{definition}[Generate and test worldviews]
    If~$G(\Pi)$ and~$T(\Pi)$ respectively are a generator and a tester program for~$\Pi$, by~$\mathit{wv}(G(\Pi), T(\Pi))$ we denote the set of all stable models~$M$ of~$G(\Pi)$ such that
    \begin{gather}
        k(M) \quad = \quad \{ ka\in K(\Pi) \mid a \in \SMC{T(\Pi); k(M)} \}.
        \label{eq:1:thm:guess-and-check}
    \end{gather}
\end{definition}




The following theorem shows that the correspondence between the worldviews of~$\Pi$ and members of~$\mathit{wv}(G(\Pi), T(\Pi))$.





\begin{theorem}\label{thm:guess-and-check}
    Let~$G(\Pi)$ be any generator program for~$\Pi$ and~$T(\Pi)$ be any tester program for~$\Pi$.
    %
    Then, there is a one\nobreakdash-to\nobreakdash-many correspondence between the worldviews of~$\Pi$ and the members of~$\mathit{wv}(G(\Pi), T(\Pi))$ such that
    \begin{enumerate}
        \item if $\wv$ is a worldview of~$\Pi$, then there is a stable model~$M$ of~$G(\Pi)$ with~$k(\wv) = k(M)$ satisfying~\eqref{eq:1:thm:guess-and-check};
        
        \item if there is a stable model~$M$ of~$G(\Pi)$ satisfying~\eqref{eq:1:thm:guess-and-check}, then the set of stable models~$\SM{T(\Pi); k(M)}$ is a worldview of~$\Pi$.
    \end{enumerate}  
\end{theorem}

\begin{proof}
Assume that~$\wv$ is a worldview of~$\Pi$.
%
By definition of worldview and tester program, it follows that 
$$\wv \ = \ \SM{\Pi^\wv} \ = \ \restr{\SM{T(\Pi); k(\wv)}}{\At{\Pi}}$$
From this and the definition of generator program,
it follows that there is a stable model~$M$ of~$G(\Pi)$ satisfying~$k(\wv) = k(M)$.
%
Futhermore, by definition of~$k(\wv)$ and the tester program, it follows that
\begin{gather}
    \begin{aligned}
        k(\wv) \ &= \ \{ ka \in K(\Pi) \mid \wv \models \K a \}
        \\
        &= \ \{ ka \in K(\Pi) \mid \restr{\SM{T(\Pi); k(\wv)}}{\At{\Pi}} \models \K a \}
        \\
        &= \ \{ ka \in K(\Pi) \mid a \in \restr{\SMC{T(\Pi); k(\wv)}}{\At{\Pi}} \}
        \\
        &= \ \{ ka \in K(\Pi) \mid a \in \SMC{T(\Pi); k(\wv)} \}
        \\
        &= \ \{ ka \in K(\Pi) \mid a \in \SMC{T(\Pi); k(M)} \}
    \end{aligned}
    \label{eq:2:thm:guess-and-check}
\end{gather}
Hence, there is a stable model~$M$ of~$G(\Pi)$ with~$k(\wv) = k(M)$ satisfying~\eqref{eq:1:thm:guess-and-check}.
\\[5pt]
Assume now that there is a stable model~$M$ of~$G(\Pi)$ satisfying~\eqref{eq:1:thm:guess-and-check} 
and take the set of stable models~$\wv = \restr{\SM{T(\Pi); k(M)}}{\At{\Pi}}$.
%
Similar to~\eqref{eq:2:thm:guess-and-check}, it follows that
\begin{gather*}
    k(\wv) \quad = \quad \{ ka\in K(\Pi) \mid a \in \SMC{T(\Pi); k(M)} \}.
\end{gather*}
and, thus, $k(\wv) = k(M)$ and~$\wv = \restr{\SM{T(\Pi); k(\wv)}}{\At{\Pi}}$.
%
By definition of tester program, it follows that~$\wv$ is a worldview of~$\Pi$.
\end{proof}

% Theorem~\ref{thm:guess-and-check} shows that, if we have any pair of generator and tester programs for a program~$\Pi$, then we can compute the worldviews of~$\Pi$ using Algorithm~\ref{alg:guess-and-check} where the fuction~\Test{$T(\Pi)$, $M$} amounts to check conditon~\eqref{eq:1:thm:guess-and-check}, and function~\BuildWorldView{$M$} amounts to compute the stable models of the tester program under assumptions~$k(M)$.







\section{Generator programs}\label{sec:reducing.candidates}

\subsection{Basic generator programs}

Let us start by showing that the tester program~$T_0(\Pi)$ is also a generator program for~$\Pi$.

\begin{proposition}\label{prop:most.basic.generator.program}
    $T_0(\Pi)$ is a generator program for~$\Pi$.
\end{proposition}

\begin{proof}
Let~$\wv$ be a worldview of~$\Pi$, that is~$\wv = \SM{\Pi^\wv}$.
%
Then,
$$
\{ M \cup k(\wv) \mid M \in \wv \} \ = \ \{ M \cup k(\wv) \mid M \in \SM{\Pi^\wv} \}
$$
%
and, by Proposition~\ref{prop:basic.tester.program}, it follows that
$$\{ M \cup k(\wv) \mid M \in \wv \} \ = \ \SM{T_0(\Pi); k(\wv)}.$$
%
Since~$\wv$ is a worldview, it is non\nobreakdash-empty and, thus, there is~$M' \in \SM{T_0(\Pi); k(\wv)}$
such that~$M' = M \cup k(\wv)$ with~$M \in \wv$.
%
Hence, $k(\wv) = k(M')$.
%
This means that~$T_0$ satisfies the first condition of Definition~\ref{def:generator.program}.

Pick now a stable model~$M$ of~$T_0(\Pi)$ and let~$\wv$ be any set of interpretations such that~$k(\wv) = k(M)$.
%
Then, 
$$M \in \SM{T_0(\Pi); k(M')} = \SM{T_0(\Pi); k(\wv)}.$$
By Corollary~\ref{cor:basic.tester.program}, it follows that~$\restr{M}{\At{\Pi}} \in \SM{\Pi^\wv}$.
%
Hence, the second condition of Definition~\ref{def:generator.program} is also satisfied.
\end{proof}

Proposition~\ref{prop:most.basic.generator.program} shows that we can use the tester program~$T_0(\Pi)$ as a generator program for~$\Pi$.
%
With some preprocessing and the differences due to the different semantics implemented in~\EPASP, this is the strategy followed by [Son et al., 2017].

[Cabalar et al., ] noted that some stable models of~$T_0(\Pi)$ can never correspond to a worldview of~$\Pi$.
%
Consider, for instance, the program\newprogramph\label{prg:most.basic.problem}
\begin{align}
    b &\leftarrow \K a
    \tag{\program{\ref{prg:most.basic.problem}}}
\end{align}
and its corresponding~$T_0(\program{\ref{prg:most.basic.problem}})$ program
\begin{align*}
    b &\leftarrow ka
    \\
    \{ ka \} &\leftarrow
\end{align*}
which has two stable models~$\emptyset$ and~$\{b, ka\}$.
%
The second stable model cannot correspond to a worldview~$\wv$ of the original program with~$k(\wv) = \{ka \}$ because
% , by the second condition in the definition of generator program, 
it correspnds to a stable model of the reduced program~$\Pi^\wv$.
%
This implies that~$\wv \not\models \K a$, which is a contradiction with~$k(\wv) = \{ka \}$.
%
Using this observation, [Cabalar et al., ] introduced a more refined generator program that reduces the number of candidates by adding constraints that ensure that the stable models of the generator program correspond that contain~$ka$ must also contain~$a$. 

By~$G_0(\Pi)$ we denote the program obtained from~$T_0(\Pi)$ by adding a constraint of the form
\begin{gather}
    \leftarrow \kk{a} \wedge \neg a
    \label{eq:consistency.constraints}
\end{gather}
for each atom~$\kk{a} \in K(\Pi)$.

Continuing with our running example, we can see that~$\{b, ka\}$ does not satisfy~\eqref{eq:consistency.constraints} and, thus, it is not a stable model of~$G_0(\program{\ref{prg:most.basic.problem}})$.
%
% Consistency constraints of the form~\eqref{eq:consistency.constraints} ensure that every stable model of the generator program correspond to an non\nobreakdash-empty set of interpretations, that is, that the second condition of Definition~\ref{def:generator.program} is satisfied.

\begin{proposition}\label{prop:basic.generator.program}
    $G_0(\Pi)$ is a generator program for~$\Pi$.
\end{proposition}

\begin{proof}
Let~$\wv$ be a worldview of~$\Pi$, that is~$\wv = \SM{\Pi^\wv}$.
%
By Proposition~\ref{prop:most.basic.generator.program}, it follows that~$T_0(\Pi)$ is a generator program for~$\Pi$ and, thus, there is a stable model~$M$ of~$T_0(\Pi)$ satisfying~$k(\wv) = k(M)$ and~$\restr{M}{\At{\Pi}} \in \wv$.
%
Pick any atom~${ka \in M}$.
%
Then, $ka \in k(M) = k(\wv)$ and, thus, $\wv \models \K a$.
%
Since~$\restr{M}{\At{\Pi}} \in \wv$, this implies that~$a \in M$ and, thus, it satisfies~\eqref{eq:consistency.constraints}.
%
Hence, $M$ is a stable model of~$G_0(\Pi)$.
%
Hence, the first condition of Definition~\ref{def:generator.program} is satisfied.

Pick now a stable model~$M$ of~$G_0(\Pi)$ and let~$\wv$ be any set of interpretations such that~$k(\wv) = k(M)$.
%
Then, $M$ is also a stable model of~$T_0(\Pi)$ and, since~$T_0(\Pi)$ is a generator program for~$\Pi$, it follows that~$\restr{M}{\At{\Pi}} \in \SM{\Pi^\wv}$.
%
Hence, the second condition of Definition~\ref{def:generator.program} is also satisfied.
\end{proof}


%
% We consider here two ways of reduing the tester checks.
%
Proposition~\ref{prop:basic.generator.program} shows that we can reduce the number of candidates by adding consistency constraints of the form of~\eqref{eq:consistency.constraints} to the generator program.
%
If we consider programs in normal form, Algorithm~\ref{alg:guess-and-check} with generator~$G_0(\Pi)$ and tester~$T_0(\Pi)$ is the core of the epistemic solver~\eclingo.
%
However, \eclingo\ does not compute the normal form of a program, so its algorithm is slightly more complicated than Algorithm~\ref{alg:guess-and-check}.
%
Hence, this a proof that on programs in normal form, \eclingo\ is correct%
%
\footnote{[Cabalar et al., ] described the algorithm of \eclingo\ but they did not show its correctness.}%
%
.

\begin{corollary}
    Algorithm~\ref{alg:guess-and-check} with generator~$G_0(\Pi)$ and tester~$T_0(\Pi)$ correctly computes the worldviews of~$\Pi$.
\end{corollary}



\subsection{Propagation of epistemic literals}

In a guess-and-check approach, the tester needs to check every stable model of the guess program.
%
Each of these checks requires a linear amount of calls to an answer set solver to compute the corresponding cautions consequences.
%
Each of these calls is coNP-complete if the program is head\nobreakdash-cycle\nobreakdash-free and $\Sigma^P_2$-complete otherwise.
%
Hence, reducing the number of tester checks is crucial to achieve a fast solver.
%
In the previous section, we saw how we can reduce the number of candidates by adding consistency constraints to the generator program.
%
In this section, we show how we can further reduce the number of candidates by propagating the consequences of epistemic literals in the generator program.


\begin{example}\label{ex:propagation}
As an example, let us consider the following program:\newprogramph\label{prg:propagation}
\begin{gather}
    \begin{aligned}
    a_i &\leftarrow \neg \K \nott{a_i} &\text{for } 0 \leq i \leq n
    \\
    \nott{a_i} &\leftarrow \neg a_i &\text{for } 0 \leq i \leq n
    \\
    g &\leftarrow a_i &\text{for } 0 \leq i \leq n
    \\
    \bot &\leftarrow \K g
\end{aligned}\tag{$\program{\ref{prg:propagation}}$}
\end{gather}
The first two rules are the result of normalizing rule~$a_i \leftarrow \neg \K \neg a_i$ usually used as a kind of subjective choice.
This program has a unique worldview~$[\emptyset]$.
%
Let us now consider its guess program~$G_0(\program{\ref{prg:propagation}})$:
\begin{align*}
    a_i &\leftarrow \neg \kknott{a_i} &\text{for } 1 \leq i \leq n
    \\
    \nott{a_i} &\leftarrow \neg a_i &\text{for } 1 \leq i \leq n
    \\
    g &\leftarrow a_i &\text{for } 0 \leq i \leq n
    \\
    \bot &\leftarrow \kk{g}
    \\
    \{ \kknott{a_i} \} &\leftarrow  &\text{for } 1 \leq i \leq n
    \\
    \{ \kk{g} \} &\leftarrow %\neg\neg \kk{g}
    \\
    \bot &\leftarrow \kknott{a_i} \wedge \neg \nott{a_i} &\text{for } 1 \leq i \leq n
    \\
    \bot &\leftarrow \kk{g} \wedge \neg g
\end{align*}
This candidate generator program has $2^{n}$ stable models of the form
$$M \cup \{ \nott{a_i} \mid a_i \notin M \} \cup \{ \kknott{a_i} \mid a_i \notin M \} \cup \{g \mid M \neq \emptyset \}$$
with~$M \subseteq \{a_1, \dotsc, a_n\}$.
%
Only the stable model corresponding to~$M = \emptyset$ leads to a worldview of the original program, while the other~$2^{n}-1$ stable models do not correspond to any worldview.
%
We can achieve an exponential speed\nobreakdash-up if we can identify the candidates that do not pass the tester check within the generator program.
%
We can observe that, in every worldview~$\wv$ of~$\program{\ref{prg:propagation}}$, if~$\wv \models \neg\K \nott{a_i}$ for any~$1 \leq i \leq n$, then every~$I \in \wv$ must satisfy~$I\models a_i$ because of the first rule.
%
Hence, every~$I \in \wv$ must satisfy~$I \models g$ because of the third rule, and we obtain~$\wv \models \K g$.
%
This contradiction the constraint~$\bot \leftarrow \K g$ and, thus, no worldview can satisfy~$\neg\K \nott{a_i}$.
%
We can achieve this reasoning within the generator program by adding rules:
\begin{align*}
    \kp{a_i} &\leftarrow \neg \kknott{a_i} &\text{for } 1 \leq i \leq n
    \\
    \kp{g} &\leftarrow \kp{a_i} &\text{for } 1 \leq i \leq n
    \\
    \bot &\leftarrow \kp{g} \wedge \neg \kk{g}
\end{align*}
The new fresh atoms~$\kp{a_i}$ and~$\kp{g}$ are respectively used to represent that~$\K a_i$ and~$\K g$ are a consequence propagated from the choices made in the generator program.
%
The meaning of~$\kp{g}$ is different from the meaning atom~$\kk{g}$ that represents the choice made in the generator program rather than an achieved consequence.
%
The unintended candidates are removed by the constraint that ensures that if conclude that~$\kp{g}$, then~$\kk{g}$ must also hold.
\end{example}

Let us now describe the general idea of the propagation of epistemic literals by introducing a new guess program~$G_1(\Pi)$.
%
For each atom~$a \in \At{\Pi}$, we introduce a new fresh atoms~$\kp{a}$ and~$\kpnott{a}$ that respectively represent that~$\K a$ and~$\K \neg a$ are consequence propagated from the choices made in the generator program.
%
We also introduce a new fresh atom~$\kpnott{r_i}$ for each rule~$r_i$ of~$\Pi$ that represents that the body of~$r_i$ is not satisfied by any interpretation of the worldview corresponding to the current candidate.
%
By~$\kp{(\Pi)}$ we denote the program containing a positive rules of the form
\begin{align}
    \kp{a_1} &\span\span\leftarrow 
    \kp{a_2},\dotsc,\kp{a_l},
    \kpnott{a_{l+1}},\dotsc,\kpnott{a_m},
    \kk{a_{m+1}},\dotsc,\kk{a_n}
    \label{eq:propagation.rule}
    \\
    \kpnott{r_i} &\leftarrow \kpnott{a_j} &&\qquad\text{for } 1 \leq j \leq l
    \\
    \kpnott{r_i} &\leftarrow \kp{a_j} &&\qquad\text{for } l+1 \leq j \leq m
    \\
    \kpnott{r_i} &\leftarrow \overline{L_j} &&\qquad\text{for } m+1 \leq j \leq n
\end{align}
for every rule~$r_i \in \Pi$ of the form
\begin{align}
    a_1 &\leftarrow 
    a_2,\dotsc,a_l,
    \neg a_{l+1},\dotsc,\neg a_m,
    \K {a_{m+1}},\dotsc,\K {a_n}
    \label{eq:propagation.rule.regular}
\end{align}
plus a rule of the form
\begin{align}
    \kpnott{a} &\leftarrow \kpnott{r_1},\dotsc,\kpnott{r_k}
    \label{eq:propagation.rule.completion}
\end{align}
for each atom~$a \in \At{\Pi}$ and where~$r_1,\dotsc,r_k$ are the rules of~$\Pi$ that have~$a$ in the head.
%
By~$G_1(\Pi)$ we denote the program obtained from~$G_0(\Pi)$ by adding the rules of~$\kp{(\Pi)}$ plus a constraints of the form
\begin{align}
    \bot &\leftarrow \kp{a} \wedge \neg \kk{a}
    \label{eq:consistency.constraints.propagation.p}
    % \\
    % \bot &\leftarrow \kpnott{a} \wedge \neg \kknott{a}
    % \label{eq:consistency.constraints.propagation.n}
\end{align}
for each atom~$\kk{a} \in K(\Pi)$.


\begin{lemma}\label{lem:propagation.generator.program}
    Let~$\wv$ be a non\nobreakdash-empty set of interpretations, and~$M$ be an interpretation such that~$k(\wv) = k(M)$.
    %
    Then,
    \begin{itemize}
        \item If~$M$ is a stable model of~$G_0(\Pi)$, then there is a unique stale model~$M'$ of~$G_0(\Pi) \cup \kp{(\Pi)}$ of the form
        $M' = M \cup M^p \cup M^n$ with
        \begin{align}
            M^p &\subseteq \{ \kp{a} \hspace{5pt} \mid \SM{\Pi^\wv} \models \K a \}
            \label{eq:1:prop:propagation.generator.program}
            \\
            M^n &\subseteq \{ \kpnott{a} \mid \SM{\Pi^\wv} \models \K \neg a \}
            \label{eq:2:prop:propagation.generator.program}
        \end{align}
        \item If $M'$ is a stable model of~$G_0(\Pi) \cup \kp{(\Pi)}$, then $M' \cap \At{G_0(\Pi)}$ is a stable model of~$G_0(\Pi)$.
    \end{itemize}
    
\end{lemma}

\begin{proof}
We use the Splitting Theorem~\cite{liftur94a}.
%
$U = \At{G_0(\Pi)}$ is a splitting set of~${G_0(\Pi) \cup \kp{(\Pi)}}$, which splitts the program into the a bottom program~$G_0(\Pi)$ and a top program~$\kp{(\Pi)}$.
%
Let~$e_U(\kp{(\Pi)},M)$ be the result of replacing in~$\kk{(\Pi)}$ each atom~$\kk{a}$ by~$\top$ if~$\kk{a} \in M$ and by~$\bot$ otherwise.
%
%
By the Splitting Theorem, $M'$ is a stable model of~$G_0(\Pi) \cup \kp{(\Pi)}$ iff there is a stable model~$M$ of~$G_0(\Pi)$ and a stable model~$M^p \cup M^n$ of~$e_U(\kp{(\Pi)},M)$ such that~$M' = M \cup M^p \cup M^n$.
%
Note that~$e_U(\kp{(\Pi)},M)$ is a Horn program and, thus, it has a unique stable model.
%
It only remains to be shown that~\eqref{eq:1:prop:propagation.generator.program} and~\eqref{eq:2:prop:propagation.generator.program} hold.
%
Since~$M^p \cup M^n$ is a stable mode of~$e_U(\kp{(\Pi)},M)$ and the latter is a Horn program, it follows that~$M^p \cup M^n = T_P^k$ for some~$k \geq 0$ whre~$T_P$ is the direct consequences operator of~$e_U(\kp{(\Pi)},M)$.
%
We prove that
\begin{align*}
    T_P^k &\subseteq 
    \{ \kp{a} \mid \SM{\Pi^\wv} \models \K a \} \cup 
    \{ \kpnott{a} \mid \SM{\Pi^\wv} \models \K \neg a \} 
    \\
    &\ \cup 
    \{ \kpnott{r_i} \mid \SM{\Pi^\wv} \models \K \neg L \text{ for some } L \in \mathit{body(r_i)} \} 
\end{align*}
for every~$k \geq 0$.
%
The proof is by induction on~$k$.
%
The case that~$k = 0$ is trivial because~$T_P^k = \emptyset$.
%
Assume now that the statement holds for~$k$ and pick~$\kp{a} \in T_P^{k+1}$.
%
Then, there is a rule~$r_i \in \Pi$ of the form of~\eqref{eq:propagation.rule.regular} such that
\begin{itemize}
    \item $\{\kp{a_2},\dotsc,\kp{a_l}\} \subseteq T_P^k$,
    \item $\{\kpnott{a_{l+1}},\dotsc,\kpnott{a_m}\} \subseteq T_P^k$,
    \item $\kk{a_i} \in M$ for all~$m+1 \leq i \leq n$.
\end{itemize}
By induction hypothsis and the fact that~$\kk{M} = \kk{\wv}$, this implies
\begin{itemize}
    \item $\SM{\Pi^\wv} \models \K a$ for all~$2 \leq i \leq l$,
    \item $\SM{\Pi^\wv} \models \K \neg a$ for all~$l+1 \leq i \leq m$,
    \item $\wv \models \K a_i$ for all~$m+1 \leq i \leq n$.
\end{itemize}
Hence, $\SM{\Pi^\wv} \models \K a$.
%
The cases for~$\kpnott{r_i} \in T_P^{k+1}$ and~$\kpnott{a} \in T_P^{k+1}$ are similar.
\end{proof}

\begin{theorem}\label{thm:propator.correctness}
    $G_1(\Pi)$ is a generator program for~$\Pi$ and, thus, Algorithm~\ref{alg:guess-and-check} with generator~$G_1(\Pi)$ and tester~$T_0(\Pi)$ correctly computes the worldviews of~$\Pi$.
\end{theorem}

\begin{proof}
Pick a worldview~$\wv$ of~$\Pi$.
%
By Proposition~\ref{prop:basic.generator.program},  there is a unique stable model~$M$ of~$G_0(\Pi)$ satisfying~$k(\wv) = k(M)$ and~$\restr{M}{\At{\Pi}} \in \wv$.
%
By Lemma~\ref{lem:propagation.generator.program}, there is a unique stable model~$M'$ of~$G_0(\Pi) \cup \kp{(\Pi)}$ of the form~$M' = M \cup M^p \cup M^n$ with~$M^p$ and~$M^n$ satisfying~\eqref{eq:1:prop:propagation.generator.program} and~\eqref{eq:2:prop:propagation.generator.program}.
%
Furthermore, $\kk(M) = \kk(M')$ and~$\restr{M'}{\At{\Pi}} = \restr{M}{\At{\Pi}} \in \wv$.
%
It only remains to be shown that~$M'$ is a stable model of~$G_1(\Pi)$, that is, that it satisfies the consistency constraints of the form of~\eqref{eq:consistency.constraints.propagation.p}.
%
Pick~$\kp{a} \in M^p$.
%
Then, $\SM{\Pi^\wv} \models \K a$ and, thus, $\wv \models \K a$ and~$\kk{a} \in M$.
%
% Similarly, for~$\kpnott{a} \in M^n$, it follows that~$\SM{\Pi^\wv} \models \K \neg a$ and, thus, $\wv \models \K \neg a$ and~$\kknott{a} \in M$.
Pick now a stable model of~$G_1(\Pi)$ and let~$\wv$ be any set of interpretations such that~$k(\wv) = k(M)$.
%
By Lemma~\ref{lem:propagation.generator.program}, $M \cap \At{G_0(\Pi)}$ is a stable model of~$G_0(\Pi)$ and, since~$G_0(\Pi)$ is a generator program for~$\Pi$, it follows that~$\restr{M}{\At{\Pi}} \in \SM{\Pi^\wv}$.
\end{proof}


Theorem~\ref{thm:propator.correctness} shows that we can use~$G_1(\Pi)$ as a generator program for~$\Pi$ instead of~$G_0(\Pi)$.
%
Let us show now that using~$G_1(\Pi)$ instead of~$G_0(\Pi)$ is actually beneficial when using Algorithm~\ref{alg:guess-and-check}.

\begin{observation}
$\mathit{s}(\kp{(\Pi)}) \leq 3 \mathit{s}(\Pi) + 2|\Pi| \leq 5 \mathit{s}(\Pi)$
and
$\mathit{s}(G_1(\Pi)) \leq 6 \mathit{s}(\Pi)$
where~$s(\cdot)$ denotes the size of a program.
\end{observation}

\begin{proposition} The following properties hold:
    \begin{enumerate}
        \item $|\SM{G_1(\Pi)}| \leq |\SM{G_0(\Pi)}|$ for every program~$\Pi$,
        \item for every program~$\Pi$ we can compute a stable mode lof $G_1(\Pi)$ from a stable model of~$G_0(\Pi)$ in linear time, and
        \item there is a family of programs~$\Pi_1, \Pi_2, \dotsc$ s.t.~$2^{i}|\SM{G_1(\Pi_i)}| \leq |\SM{G_0(\Pi_i)}|$ and~$\mathcal{O}(s(\Pi_i)) = i$.
    \end{enumerate}
\end{proposition}

\begin{proof}
By Lemma~\ref{lem:propagation.generator.program}, 
it follows that~$|\SM{G_0(\Pi)\cup \kp{(\Pi)}}| = |\SM{G_0(\Pi)}|$.
%
Since~$G_1(\Pi)$ is the result of adding some integrity constrains to~$G_0(\Pi) \cup \kp{(\Pi)}$, the first property holds.
%
For the second property, we can compute a stable model~$M$ of~$G_0(\Pi)\cup kp{(\Pi)}$ from a stable model~$M'$ of~$G_0(\Pi)$ by adding the consequences~$e_U(\kp{(\Pi)},M')$.
%
Since this is a definite program, its consequence can be computed in linear time.
%
Checking that the constraints in~$G_1(\Pi) \setminus G_1(\Pi)\cup kp{(\Pi)}$ are satisfied also can be computed in linear time.
%
Finally, for the third property, consider the program~$\Pi_i$ of Example~\ref{ex:propagation}.
\end{proof}

The first two properties show that using~$G_1(\Pi)$ instead of~$G_0(\Pi)$ only incurs a linear overhead in computing the stable models of the generator program.
%
In particular, the first property ensures that the loop in between lines~\ref{alg.generator.loop.ini} and~\ref{alg.generator.loop.end} of Algorithm~\ref{alg:guess-and-check} is never required to do more iteratrions when using~$G_1(\Pi)$ instead of~$G_0(\Pi)$.
%
The third property shows that using~$G_1(\Pi)$ can reduce the number of candidates that need to be checked exponentially.




% never increases the number of candidates that need to be checked and only incurs a polynomial overhead in the generator program.

% %
% Example~\ref{ex:propagation} shows that in some cases the number of candidates that need to be checked can be reduced exponentially by using~$G_1(\Pi)$ instead of~$G_0(\Pi)$.


% \begin{proposition}\label{prop:propagation.generator.program}
%     Let~$\wv$ be a non\nobreakdash-empty set of interpretations and~$M$ be a stable model of~$G_0(\Pi) \cup \kp{(\Pi)}$ such that~$k(\wv) = k(M)$.
%     %
%     Then,
%     $pk{a} \in M$ implies that~$\SM{\Pi^\wv} \models \K a$
%     and
%     $\kpnott{a} \in M$ implies that~$\SM{\Pi^\wv} \models \K \neg a$.
% \end{proposition}

% \begin{proof}

% \end{proof}

% \subsection{Consistency constraints}\label{sec:consistency.constraints}

% Consider the program~$\Pi$
% \begin{align*}
%     a &\leftarrow \neg \K \neg a 
%     \\
%     b_i &\leftarrow a     &\text{for } 1 \leq i \leq n
%     \\
%     c &\leftarrow \K b_i  &\text{for } 1 \leq i \leq n
%     \\
%     \bot &\leftarrow \neg c
% \end{align*}
% This program has a unique worldview~$[\{a, b_0, \dotsc, b_n, c\}]$.
% %
% Let us now consider its guess program~$G_0(\Pi)$:
% \begin{align*}
%     a &\leftarrow \neg \kk{na}
%     \\
%     na &\leftarrow \neg a
%     \\
%     b_i &\leftarrow a_i &\text{for } 1 \leq i \leq n
%     \\
%     c &\leftarrow kb_i  &\text{for } 1 \leq i \leq n
%     \\
%     \bot &\leftarrow \neg c
%     \\
%     \{\kk{b_i}\} &\leftarrow &\text{for } 1 \leq i \leq n
%     \\
%     \bot &\leftarrow \kk{b_i} \wedge \neg b_i &\text{for } 1 \leq i \leq n
% \end{align*}
% This candidate generator program has $2^{n}-1$ stable models, among which only one of them correspondens to the serched worldview.
% %
% This means that, in the world case scenario, the tester  needs to check~$2^n-2$ candidates before finding a worldview.



% \newpage

% \begin{align*}
%     a_i &\leftarrow \neg \K \neg a_i &\text{for } 0 \leq i \leq n
%     \\
%     \{ g \} &\leftarrow
%     \\
%     g &\leftarrow a_1 \wedge \dotsb \wedge a_n
%     \\
%     \bot &\leftarrow \K \neg g
% \end{align*}
% This program has a unique worldview~$[\{a_0, \dotsc, a_n, g\}]$.
% %
% Let us now consider its guess program~$G_0(\Pi)$:
% \begin{align*}
%     a_i &\leftarrow \neg \kk{a_i}' &\text{for } 1 \leq i \leq n
%     \\
%     a_i' &\leftarrow \neg a_i &\text{for } 1 \leq i \leq n
%     \\
%     g &\leftarrow \neg\neg g
%     \\
%     g &\leftarrow a_0 \wedge \dotsb \wedge a_n
%     \\
%     \bot &\leftarrow \neg \kk{g}
%     \\
%     \kk{a_i'} &\leftarrow \neg\neg \kk{a_i'} &\text{for } 1 \leq i \leq n
%     \\
%     \kk{g} &\leftarrow \neg\neg \kk{g}
%     \\
%     \bot &\leftarrow \kk{a_i'} \wedge \neg a_i' &\text{for } 1 \leq i \leq n
%     \\
%     \bot &\leftarrow \kk{g} \wedge \neg g
% \end{align*}
% This candidate generator program has $2^{n}$ stable models.
% %
% Each of these stable models either contains~$a_i$ or~$\kk{a_i'}$ for each~$0 \leq i \leq n$.

% needs to be checked by the tester.



% The first line of the program guess the actions, the second line is an effect of those actions, and the third line states that the goal must be satisfied.
% %
% Obiously, in a real conformant planning problem, we will have inertia axioms and more involving model of the effects of actions.




% We can reduce the number of candidates that need to be checked by propagating the some consequences in the guess program.
% %
% For instance,
% consider the program and, its associdated guess program
% \begin{gather*}
%     \begin{aligned}[t]
%         a_0 &\leftarrow \neg \K b
%         \\
%         b &\leftarrow \neg a
%         \\
%         a_{i+1} &\leftarrow \K a_i &\text{for } 0 \leq i < n
%     \end{aligned}
%     \hspace{2cm}
%     \begin{aligned}[t]
%         a_0 &\leftarrow \neg kb
%         \\
%         b &\leftarrow \neg a_0
%         \\
%         a_{i+1} &\leftarrow ka_i &\text{for } 0 \leq i < n
%         \\
%         ka_i &\leftarrow \neg\neg ka_i &\text{for } 0 \leq i < n
%         \\
%         \bot &\leftarrow ka_i \wedge \neg a_i &\text{for } 0 \leq i < n
%     \end{aligned}
% \end{gather*}
% This programs has two worldviews~$[\{b\}]$ and~$[\{a_0, a_1, \dotsc, a_n \}]$.
% %
% The associdated guess program has $n+1$ stable models
% $\{b \}$, $\{a_0 \}$, $\{a_0, k_0, a_1 \}$, $\{a_0, k_0, a_1, k_1, a_2 \}$, $\dotsc$
% $\{a_0, k_0, a_1, k_1, \dotsc, a_n\}$ that need to be checked by the tester.
% %
% Each of those checks being a coNP-hard problem.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

\url{potassco.org}


==> implementation.tex <==
\section{Implementation}


We implemented a new solver for epistemic logic programs based on Algorithm~\ref{alg:guess-and-check}.
%
Our implementation is built on top of version~5.7 of the ASP solver~\texttt{clingo} solver~\cite{gekakasc17a} using its Python API\footnote{\url{https://potassco.org/clingo/python-api/5.7/}}.
%
We extend the language of \texttt{clingo} by allowing literals of the form $\texttt{\&k\{} L \texttt{\}}$ in the body of rules, with $L$ being a literal of the forms~$A$, $\texttt{not\,}A$, or $\texttt{not\,not\,} A$ for some atom~$A$ in the usual syntax of~\texttt{clingo}.
%
Once this is added as an external theory to \texttt{clingo}, it handles the parsing leaving us to focus only on the implementation of the epistemic solver.
%
An interesting side effect of this approach is that our solver accepts all the features of \texttt{clingo} such as aggregates, choice rules, intervals, pools, etc.
%
The first step after parsing consists of computing the normal form of the non\nobreakdash-ground program and rewriting it as a non\nobreakdash-epistemic program that we can ground using \texttt{clingo} as well as using the result after grounding to reconstruct the epistemic program.
%
For instance, rule
\small
\begin{flalign*}
    &\texttt{a,\,b\,:-\,c(X),\,not\,\&k\{\,not\, d(X)\,\}.}
\end{flalign*}
\normalsize
is translated as the non\nobreakdash-epistemic rules:
\small
\begin{flalign}
    &\texttt{u(a),\,u(b) :-\,u(c(X)),\,not\,k(not1(d(X))).}
    \label{eq:non-epistemic.r1}
    \\
    &\texttt{not1(d(X))\,:-\,u(c(X)),\,not\,d(X).}
\end{flalign}
\normalsize
where predicate symbol~$k/1$ represents the epistemic operator~$\K$ and~$u/1$ is a unary predicate used to avoid name collisions.
%
Atom~$\texttt{k(not1(d(X)))}$ is used to compute the normal form.
%
In addition, choice rule
\small
\begin{flalign*}
    &\texttt{\{k(not1(d(X)))\} :- not1(d(X)).}
\end{flalign*}
\normalsize
is added to ensure the grounding of the non\nobreakdash-epistemic program matches the grounding of the epistemic program.


One important aspect of our implementation is that it easily allows us to use different guess and check programs.
%
To achieve this, we rely on \emph{metaprogramming}, where the ground program is reified as a set of facts and we can use an ASP program to produce the generator and check programs~\cite{karoscwa21a}.
%
This allows us to change the generator and test programs by only changing the ASP metaprogram.
%
For instance, if we add the fact~$\texttt{c(1)}$ to rule~\eqref{eq:non-epistemic.r1}, we may obtain the following set of facts:
\small
\begin{flalign*}
    & \texttt{rule(disjunction(1),\,normal(2)).}
    \\
    & \texttt{atom\_tuple(1).}
    \\
    & \texttt{atom\_tuple(1,3). atom\_tuple(1,4).}
    \\
    &\texttt{literal\_tuple(2).}
    \\
    &\texttt{literal\_tuple(2,5). literal\_tuple(2,-6).}
\end{flalign*}
\normalsize
The first fact indicates that rule~\eqref{eq:non-epistemic.r1} is a disjunction rule with a normal body.
%
Alternatively, it could be a choice rule or have a weighted body representing a sum aggregate.
%
The number one in the first argument of the fact in the first line indicates the $\mathit{atom\_tuple}$ that represents the head.
%
In this case, it contains two atoms,~$a$ and~$b$, coded as the numbers~$3$ and~$4$, respectively.
%
This is encoded in lines~2 and~3.
%
Finally, the number two in the second argument of the fact in the first line indicates the $\mathit{literal\_tuple}$ that represents the body.
%
This contains two literals,~$\texttt{c(1)}$ and~$\texttt{k(no1(d(1)))}$, coded as the numbers~$5$ and~$6$, respectively.
%
The negative sign indicates that the literal is negated.
%
Using this representation, we can generate all rules of the form of~\eqref{eq:propagation.rule.regular} using the metarules in Figure~\ref{fig:metarules}.
%
Atom~$\mathit{hold(n)}$ represents that the atom identified by code~$n$ is true.
%
Atoms~$\mathit{kp\_hold(n)}$ and~$\mathit{kp\_not\_hold(n)}$ correspond to the atoms of the form of~$\kp{a}$ and~$\kpnott{a}$ for atom~$a$ with code~$n$, respectively.
%
Predicate~$\mathit{epistemic\_atom}$ is used to identify codes that correspond to epistemic literals.
%
The first rule in Figure~\ref{fig:metarules} makes atom~$\mathit{kp\_body(b)}$ true when the body~$b$ holds.
%
The second rule makes some atom~$\mathit{kp\_hold(a)}$ in the head of the disjunctive rule true with body~$b$ when this holds.

==> metarulesfig.tex <==
\begin{figure*}[t]
    \small
    \begin{flalign*}
        \\
        &\texttt{kp\_body(B) :- literal\_tuple(B),}
        \\
        &\hspace*{104pt}\texttt{kp\_hold(A)\,:\,literal\_tuple(B,\phantom{-}A),  A > 0, not epistemic\_atom(A);
        }
        \\
        &\hspace*{118pt}\texttt{hold(A)\,:\,literal\_tuple(B,\phantom{-}A),  A > 0,     epistemic\_atom(A);
        }
        \\
        &\hspace*{80pt}\texttt{
            kp\_not\_hold(A)\,:\,literal\_tuple(B,-A), A > 0, not epistemic\_atom(A);
        }
        \\
        &\hspace*{92pt}\texttt{
               not hold(A)\,:\,literal\_tuple(B,-A), A > 0,     epistemic\_atom(A).
        }
        \\
        &\texttt{kp\_hold(A) : atom\_tuple(H,A) :- rule(disjunction(H), B), kp\_body(B).}
    \end{flalign*}
    \caption{Metarules to generate the rules of the form of~\eqref{eq:propagation.rule.regular}.}\label{fig:metarules}
\end{figure*}

==> preprocessing.tex <==
\section{Preprocessing}

[Son et al., 2017] introduced a preprocessing step to reduce the number of candidates provided by the guess program.
%
This consists on fixing the values of the atoms of the form~$\kk{a}$ according to the cautions of the basic program.
%
This preprocessing can be improved in two ways.
%
First, we can iterate this process until reaching a fix point.
%
For instance, let us consider the program and, its associated basic program
\begin{gather*}
    \begin{aligned}[t]
        a &\leftarrow \neg\neg a
        \\
        \bot &\leftarrow \neg a
        \\
        b &\leftarrow \K a
        \\
        c &\leftarrow \K b
    \end{aligned}
    \hspace{2cm}
    \begin{aligned}[t]
        a &\leftarrow \neg\neg a
        \\
        \bot &\leftarrow \neg a
        \\
        b &\leftarrow ka
        \\
        c &\leftarrow kb
        \\
        ka &\leftarrow \neg\neg ka
        \\
        kb &\leftarrow \neg\neg kb
    \end{aligned}
\end{gather*}
The cautions consequences of the basic program is set~$\{ a \}$.
%
The preprocessing step fixes the value of~$ka$ by adding rule~$\neg\neg ka$ to the program.
%
The cautions consequences of the basic program is set~$\{ a, b \}$ and the preprocessing step fixes the value of~$kb$ by adding rule~$\neg\neg kb$ to the program.
%
The cautions consequences of the basic program is set~$\{ a, b, c \}$.


Computing the cautions consequences of a program is coNP complete.
%
We can replace this step by approximating the cautions consequences in polynomial time and only computing the cautions consequences of the basic program once the approximation reaches a fix point.

An \emph{cautious consequences approximation}~$\SMCA{\Pi} = (L,U)$ of a program~$\Pi$ is a pair of sets of atoms such that~$L \subseteq \SMC{\Pi} \subseteq U$.

\begin{theorem}
    Let~$T(\Pi)$ be any test program for~$\Pi$ and let~$\SMCA{T(\Pi)} = (L,U)$ be any cautious consequences approximation of~$T(\Pi)$.
    %
    Then, 
    \begin{gather*}
        T(\Pi) \cup \{ \neg\neg ka \mid a \in L \cap \At{\Pi} \} \cup \{ \neg ka \mid a \in \At{\Pi} \setminus U \}
    \end{gather*}
    is also a test program of~$\Pi$.
\end{theorem}


\begin{theorem}
    Let~$G(\Pi)$ be any guest program for~$\Pi$ and let~$\SMCA{T(\Pi)} = (L,U)$ be any cautious consequences approximation of a test program~$T(\Pi)$ for~$\Pi$.
    %
    Then, 
    \begin{gather*}
        G(\Pi) \cup \{ \neg\neg ka \mid a \in L \cap \At{\Pi} \} \cup \{ \neg ka \mid a \in \At{\Pi} \setminus U \}
    \end{gather*}
    is also a guess program of~$\Pi$.
\end{theorem}

==> solver_comp_eclingo.tex <==
\addplot[
    dashed,
    color=green,
    mark=*,
    ]
    coordinates {
        (1,0.082662)(2,0.0831845)(3,0.0833445)(4,0.0833705)(5,0.08457049999999999)(6,0.0848215)(7,0.084984)(8,0.0862875)(9,0.086501)(10,0.087004)(11,0.0874515)(12,0.087807)(13,0.0879065)(14,0.087922)(15,0.0880055)(16,0.08891399999999999)(17,0.0896905)(18,0.0902195)(19,0.0907735)(20,0.0912965)(21,0.09182)(22,0.0935155)(23,0.0935485)(24,0.093977)(25,0.094224)(26,0.094467)(27,0.09461800000000001)(28,0.0947105)(29,0.09559300000000001)(30,0.0965305)(31,0.0974435)(32,0.09819249999999999)(33,0.098495)(34,0.10149749999999999)(35,0.10213900000000001)(36,0.10734199999999999)(37,0.107757)(38,0.108198)(39,0.110652)(40,0.116497)(41,0.11683750000000001)(42,0.12095700000000001)(43,0.1212935)(44,0.13688699999999998)(45,0.1375665)(46,0.14170549999999998)(47,0.15276450000000003)(48,0.1604825)(49,0.1667415)(50,0.218474)(51,0.235753)(52,0.2503865)(53,0.33779349999999997)(54,0.349786)(55,0.3843665)(56,0.4057265)(57,0.4113945)(58,0.43431949999999997)(59,0.4657545)(60,0.514817)(61,0.562808)(62,0.5675479999999999)(63,0.6242505)(64,0.713753)(65,0.8287015)(66,0.830163)(67,0.8623719999999999)(68,0.9288915)(69,0.9914480000000001)(70,1.1481599999999998)(71,1.7825199999999999)(72,1.915895)(73,1.91915)(74,1.926295)(75,2.0416)(76,2.11333)(77,2.116705)(78,2.3074250000000003)(79,2.38796)(80,2.651985)(81,3.386)(82,4.031855)(83,4.1553450000000005)(84,4.425585)(85,4.579845000000001)(86,5.63999)(87,5.696009999999999)(88,5.804365)(89,5.965145)(90,6.923445)(91,7.276)(92,7.694355)(93,7.774240000000001)(94,8.5379)(95,8.62839)(96,9.03755)(97,9.31514)(98,9.900110000000002)(99,10.4409)(100,11.04005)(101,11.1395)(102,11.66215)(103,15.418199999999999)(104,15.938399999999998)(105,16.6226)(106,18.34385)(107,19.83915)(108,22.9127)(109,23.274250000000002)(110,26.9637)(111,27.5066)(112,28.5473)(113,29.488500000000002)(114,30.3283)(115,31.64)(116,34.060199999999995)(117,43.73015)(118,54.560050000000004)(119,61.6233)(120,63.69584999999999)(121,78.60974999999999)(122,87.1776)(123,91.82005)(124,106.906)(125,107.232)(126,112.768)(127,141.7865)(128,152.887)(129,169.9865)(130,177.3405)(131,211.687)(132,222.51999999999998)(133,308.89)(134,336.8235)(135,352.12800000000004)(136,393.4995)(137,426.6805)(138,474.66999999999996)(139,484.2925)(140,501.985)(141,516.5160000000001)(142,578.5364999999999)(143,586.948)(144,588.4205)(145,591.1700000000001)(146,591.7785)(147,594.927)(148,595.6645)(149,595.745)(150,597.1179999999999)(151,597.578)(152,597.5835)(153,597.585)(154,598.3895)(155,598.5805)(156,598.6205)(157,598.9955)(158,599.2265)(159,599.4365)(160,599.694)(161,599.7065)(162,600.0)(163,600.0)(164,600.0)(165,600.0)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
    \addlegendentry{ \texttt{eclingo} }

==> solver_comp_elp2qasp.tex <==
\addplot[
dotted,
color=violet,
mark=x,
]
coordinates {
        (1,0.6788974999999999)(2,0.757239)(3,1.04672)(4,1.257165)(5,1.3538450000000002)(6,1.504585)(7,1.729625)(8,2.0452399999999997)(9,2.242965)(10,2.63274)(11,2.647905)(12,2.69453)(13,2.76502)(14,3.20118)(15,3.797325)(16,3.831725)(17,5.52142)(18,5.971285)(19,19.81545)(20,36.95515)(21,263.288)(22,600.0)(23,600.0)(24,600.0)(25,600.0)(26,600.0)(27,600.0)(28,600.0)(29,600.0)(30,600.0)(31,600.0)(32,600.0)(33,600.0)(34,600.0)(35,600.0)(36,600.0)(37,600.0)(38,600.0)(39,600.0)(40,600.0)(41,600.0)(42,600.0)(43,600.0)(44,600.0)(45,600.0)(46,600.0)(47,600.0)(48,600.0)(49,600.0)(50,600.0)(51,600.0)(52,600.0)(53,600.0)(54,600.0)(55,600.0)(56,600.0)(57,600.0)(58,600.0)(59,600.0)(60,600.0)(61,600.0)(62,600.0)(63,600.0)(64,600.0)(65,600.0)(66,600.0)(67,600.0)(68,600.0)(69,600.0)(70,600.0)(71,600.0)(72,600.0)(73,600.0)(74,600.0)(75,600.0)(76,600.0)(77,600.0)(78,600.0)(79,600.0)(80,600.0)(81,600.0)(82,600.0)(83,600.0)(84,600.0)(85,600.0)(86,600.0)(87,600.0)(88,600.0)(89,600.0)(90,600.0)(91,600.0)(92,600.0)(93,600.0)(94,600.0)(95,600.0)(96,600.0)(97,600.0)(98,600.0)(99,600.0)(100,600.0)(101,600.0)(102,600.0)(103,600.0)(104,600.0)(105,600.0)(106,600.0)(107,600.0)(108,600.0)(109,600.0)(110,600.0)(111,600.0)(112,600.0)(113,600.0)(114,600.0)(115,600.0)(116,600.0)(117,600.0)(118,600.0)(119,600.0)(120,600.0)(121,600.0)(122,600.0)(123,600.0)(124,600.0)(125,600.0)(126,600.0)(127,600.0)(128,600.0)(129,600.0)(130,600.0)(131,600.0)(132,600.0)(133,600.0)(134,600.0)(135,600.0)(136,600.0)(137,600.0)(138,600.0)(139,600.0)(140,600.0)(141,600.0)(142,600.0)(143,600.0)(144,600.0)(145,600.0)(146,600.0)(147,600.0)(148,600.0)(149,600.0)(150,600.0)(151,600.0)(152,600.0)(153,600.0)(154,600.0)(155,600.0)(156,600.0)(157,600.0)(158,600.0)(159,600.0)(160,600.0)(161,600.0)(162,600.0)(163,600.0)(164,600.0)(165,600.0)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
\addlegendentry{\texttt{elp2qasp}}

==> solver_comp_epasp.tex <==
\addplot[
    dashed,
    color=yellow,
    mark=x,
    ]
    coordinates {
        (1,0.001571)(2,0.008602499999999999)(3,0.009071)(4,0.012036999999999999)(5,0.015216)(6,0.0156585)(7,0.0156585)(8,0.0156585)(9,0.02972)(10,0.09093899999999999)(11,0.090964)(12,0.09231600000000001)(13,0.09399550000000001)(14,0.09633749999999999)(15,0.097559)(16,0.10023)(17,0.10125)(18,0.1073625)(19,0.10890050000000001)(20,0.11887600000000001)(21,0.129986)(22,0.138416)(23,0.14647949999999998)(24,0.15289799999999998)(25,0.153177)(26,0.1549975)(27,0.1613075)(28,0.18138100000000001)(29,0.182256)(30,0.185805)(31,0.1898235)(32,0.190066)(33,0.2918535)(34,0.3604)(35,0.3625795)(36,0.37163500000000005)(37,0.39266650000000003)(38,0.415846)(39,0.4331955)(40,0.503023)(41,0.5208124999999999)(42,0.659082)(43,0.668829)(44,0.6939915)(45,1.0067205000000001)(46,1.097325)(47,1.2383899999999999)(48,1.30443)(49,1.427545)(50,1.777155)(51,1.93245)(52,2.060285)(53,2.07011)(54,2.35268)(55,2.4309000000000003)(56,2.8895299999999997)(57,3.135085)(58,3.27035)(59,3.4832)(60,3.683225)(61,4.557295)(62,4.86781)(63,4.98204)(64,5.285905)(65,5.337695)(66,7.34757)(67,7.844234999999999)(68,8.480595000000001)(69,8.882615000000001)(70,10.42)(71,10.59535)(72,10.9185)(73,14.444600000000001)(74,15.455950000000001)(75,15.6878)(76,19.33175)(77,20.43385)(78,20.79965)(79,24.502299999999998)(80,24.86385)(81,25.2709)(82,27.154)(83,32.46835)(84,35.224199999999996)(85,36.6045)(86,37.29345)(87,37.52235)(88,40.977450000000005)(89,43.1949)(90,50.36805)(91,51.25925)(92,54.046400000000006)(93,55.760999999999996)(94,70.8968)(95,74.87525)(96,76.40520000000001)(97,90.53165000000001)(98,93.6799)(99,107.758)(100,120.9585)(101,157.3875)(102,197.547)(103,204.172)(104,220.253)(105,305.5425)(106,334.64099999999996)(107,352.45500000000004)(108,352.457)(109,359.1355)(110,387.92150000000004)(111,409.446)(112,412.5855)(113,440.3635)(114,474.86)(115,480.818)(116,489.6075)(117,559.0)(118,559.3405)(119,581.789)(120,591.3720000000001)(121,594.5195)(122,594.7495)(123,595.4855)(124,596.4970000000001)(125,600.0)(126,600.0)(127,600.0)(128,600.0)(129,600.0)(130,600.0)(131,600.0)(132,600.0)(133,600.0)(134,600.0)(135,600.0)(136,600.0)(137,600.0)(138,600.0)(139,600.0)(140,600.0)(141,600.0)(142,600.0)(143,600.0)(144,600.0)(145,600.0)(146,600.0)(147,600.0)(148,600.0)(149,600.0)(150,600.0)(151,600.0)(152,600.0)(153,600.0)(154,600.0)(155,600.0)(156,600.0)(157,600.0)(158,600.0)(159,600.0)(160,600.0)(161,600.0)(162,600.0)(163,600.0)(164,600.0)(165,600.0)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
\addlegendentry{$\texttt{EP-ASP}^{\mathit{se}}$}


==> solver_comp_epasp_noplanning.tex <==
\addplot[
        color=violet,
        mark=x,
        ]
        coordinates {
        (1,0.031178)(2,0.032090499999999994)(3,0.033447500000000005)(4,0.0337985)(5,0.034213)(6,0.0345305)(7,0.035324)(8,0.0353975)(9,0.0363715)(10,0.0374455)(11,0.039135500000000004)(12,0.039166)(13,0.040163500000000005)(14,0.0422255)(15,0.0476365)(16,0.05848)(17,0.07842450000000001)(18,0.09093899999999999)(19,0.090964)(20,0.09231600000000001)(21,0.09399550000000001)(22,0.10890050000000001)(23,0.125077)(24,0.1549975)(25,0.1679805)(26,0.178454)(27,0.182256)(28,0.1898235)(29,0.206745)(30,0.2478885)(31,0.313266)(32,0.465581)(33,0.503843)(34,0.506104)(35,0.5208124999999999)(36,0.8379369999999999)(37,0.9469165)(38,1.0719699999999999)(39,1.2353999999999998)(40,1.67059)(41,1.777155)(42,2.10996)(43,2.4309000000000003)(44,3.135085)(45,3.759845)(46,4.557295)(47,37.52235)(48,51.25925)(49,97.27635000000001)(50,115.178)(51,162.2465)(52,163.074)(53,169.0085)(54,176.154)(55,187.624)(56,195.91449999999998)(57,198.822)(58,239.502)(59,246.331)(60,267.1975)(61,282.8325)(62,305.5425)(63,313.22)(64,315.86400000000003)(65,334.64099999999996)(66,352.073)(67,352.45500000000004)(68,359.1355)(69,387.92150000000004)(70,396.42949999999996)(71,409.446)(72,412.5855)(73,440.3635)(74,448.235)(75,474.86)(76,480.818)(77,489.6075)(78,556.674)(79,559.0)(80,559.3405)(81,581.789)(82,600.0)(83,600.0)(84,600.0)(85,600.0)(86,600.0)(87,600.0)(88,600.0)(89,600.0)(90,600.0)(91,600.0)(92,600.0)(93,600.0)(94,600.0)(95,600.0)(96,600.0)(97,600.0)(98,600.0)(99,600.0)(100,600.0)(101,600.0)(102,600.0)(103,600.0)(104,600.0)(105,600.0)(106,600.0)(107,600.0)(108,600.0)(109,600.0)(110,600.0)(111,600.0)(112,600.0)(113,600.0)(114,600.0)(115,600.0)(116,600.0)(117,600.0)(118,600.0)(119,600.0)(120,600.0)(121,600.0)(122,600.0)(123,600.0)(124,600.0)(125,600.0)(126,600.0)(127,600.0)(128,600.0)(129,600.0)(130,600.0)(131,600.0)(132,600.0)(133,600.0)(134,600.0)(135,600.0)(136,600.0)(137,600.0)(138,600.0)(139,600.0)(140,600.0)(141,600.0)(142,600.0)(143,600.0)(144,600.0)(145,600.0)(146,600.0)(147,600.0)(148,600.0)(149,600.0)(150,600.0)(151,600.0)(152,600.0)(153,600.0)(154,600.0)(155,600.0)(156,600.0)(157,600.0)(158,600.0)(159,600.0)(160,600.0)(161,600.0)(162,600.0)(163,600.0)(164,600.0)(165,600.0)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
\addlegendentry{$\texttt{EP-ASP}$}

==> solver_comp_g0.tex <==
\addplot[
    color=red,
    mark=x,
    ]
    coordinates {
        (1,0.0)(2,0.0)(3,0.0)(4,0.0)(5,0.001)(6,0.001)(7,0.001)(8,0.001)(9,0.001)(10,0.001)(11,0.001)(12,0.001)(13,0.001)(14,0.001)(15,0.001)(16,0.001)(17,0.001)(18,0.001)(19,0.001)(20,0.001)(21,0.001)(22,0.001)(23,0.0015)(24,0.0015)(25,0.002)(26,0.002)(27,0.002)(28,0.002)(29,0.002)(30,0.002)(31,0.002)(32,0.002)(33,0.003)(34,0.004)(35,0.004)(36,0.004)(37,0.005)(38,0.005)(39,0.0055)(40,0.007)(41,0.007)(42,0.007)(43,0.0075)(44,0.008)(45,0.008)(46,0.008)(47,0.008)(48,0.009)(49,0.010499999999999999)(50,0.011)(51,0.013)(52,0.013)(53,0.014)(54,0.014)(55,0.017)(56,0.018)(57,0.018000000000000002)(58,0.02)(59,0.02)(60,0.022)(61,0.024)(62,0.027)(63,0.033)(64,0.036)(65,0.0375)(66,0.039)(67,0.0405)(68,0.044)(69,0.0465)(70,0.053)(71,0.053500000000000006)(72,0.064)(73,0.0645)(74,0.0715)(75,0.082)(76,0.08499999999999999)(77,0.087)(78,0.088)(79,0.0885)(80,0.092)(81,0.094)(82,0.095)(83,0.098)(84,0.1005)(85,0.1115)(86,0.127)(87,0.128)(88,0.129)(89,0.135)(90,0.1495)(91,0.1525)(92,0.157)(93,0.165)(94,0.166)(95,0.178)(96,0.181)(97,0.191)(98,0.209)(99,0.2185)(100,0.2215)(101,0.255)(102,0.262)(103,0.279)(104,0.2795)(105,0.295)(106,0.2985)(107,0.3095)(108,0.37)(109,0.40049999999999997)(110,0.4435)(111,0.5335000000000001)(112,0.538)(113,0.642)(114,0.647)(115,0.6685000000000001)(116,0.6795)(117,0.715)(118,0.887)(119,0.967)(120,1.021)(121,1.0495)(122,1.097)(123,1.202)(124,1.3615)(125,1.385)(126,1.5845)(127,1.956)(128,2.324)(129,2.572)(130,2.5865)(131,2.6615)(132,3.304)(133,3.8135)(134,4.407)(135,4.884)(136,4.9185)(137,5.8315)(138,5.94)(139,6.391)(140,6.656000000000001)(141,7.235)(142,8.084499999999998)(143,9.374)(144,9.563500000000001)(145,9.604)(146,9.994)(147,11.94)(148,12.325)(149,12.574)(150,13.189499999999999)(151,19.247500000000002)(152,19.299)(153,21.976)(154,22.747)(155,22.911)(156,25.759)(157,27.314)(158,32.3605)(159,37.239)(160,37.460499999999996)(161,43.175)(162,51.040499999999994)(163,60.0795)(164,182.252)(165,548.401)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
\addlegendentry{ $G_0$ }

==> solver_comp_g1.tex <==
\addplot[
    color=blue,
    mark=*,
    ]
    coordinates {
    %     (1,0.0)(2,0.0)(3,0.001)(4,0.001)(5,0.001)(6,0.001)(7,0.001)(8,0.001)(9,0.002)(10,0.002)(11,0.002)(12,0.002)(13,0.002)(14,0.002)(15,0.003)(16,0.003)(17,0.003)(18,0.003)(19,0.0035)(20,0.004)(21,0.004)(22,0.004)(23,0.004)(24,0.0045000000000000005)(25,0.0055)(26,0.0055)(27,0.007)(28,0.0075)(29,0.0075)(30,0.0075)(31,0.008)(32,0.008)(33,0.0085)(34,0.009)(35,0.009)(36,0.0095)(37,0.0095)(38,0.01)(39,0.01)(40,0.011)(41,0.012)(42,0.013)(43,0.014)(44,0.014)(45,0.014499999999999999)(46,0.015)(47,0.016)(48,0.016)(49,0.0165)(50,0.017)(51,0.017)(52,0.017)(53,0.018)(54,0.0185)(55,0.019)(56,0.0195)(57,0.02)(58,0.02)(59,0.022)(60,0.022)(61,0.0225)(62,0.0245)(63,0.025)(64,0.025500000000000002)(65,0.026)(66,0.0265)(67,0.027)(68,0.0275)(69,0.0285)(70,0.029)(71,0.029)(72,0.0295)(73,0.0305)(74,0.035500000000000004)(75,0.0365)(76,0.0405)(77,0.041)(78,0.041999999999999996)(79,0.041999999999999996)(80,0.0435)(81,0.0435)(82,0.045)(83,0.0455)(84,0.046)(85,0.0495)(86,0.0495)(87,0.051500000000000004)(88,0.0545)(89,0.057)(90,0.058499999999999996)(91,0.073)(92,0.0745)(93,0.081)(94,0.0825)(95,0.089)(96,0.0925)(97,0.0965)(98,0.098)(99,0.1005)(100,0.1015)(101,0.1035)(102,0.1095)(103,0.119)(104,0.1395)(105,0.14150000000000001)(106,0.143)(107,0.14400000000000002)(108,0.14550000000000002)(109,0.15)(110,0.162)(111,0.16599999999999998)(112,0.166)(113,0.1735)(114,0.183)(115,0.186)(116,0.187)(117,0.1995)(118,0.209)(119,0.2285)(120,0.23299999999999998)(121,0.2425)(122,0.2525)(123,0.2735)(124,0.3035)(125,0.31)(126,0.325)(127,0.332)(128,0.33399999999999996)(129,0.335)(130,0.3865)(131,0.4165)(132,0.443)(133,0.473)(134,0.511)(135,0.5615)(136,0.576)(137,0.5905)(138,0.699)(139,0.6995)(140,0.709)(141,0.713)(142,0.767)(143,0.7705)(144,0.7945)(145,0.873)(146,0.9430000000000001)(147,1.093)(148,1.209)(149,1.476)(150,1.492)(151,1.6244999999999998)(152,1.669)(153,1.9645)(154,2.074)(155,2.433)(156,2.656)(157,2.7105)(158,2.7554999999999996)(159,2.791)(160,3.2279999999999998)(161,3.426)(162,3.4875)(163,3.7359999999999998)(164,3.945)(165,5.074)(166,5.6205)(167,5.6835)(168,6.1739999999999995)(169,6.858499999999999)(170,7.101)(171,7.1845)(172,7.401)(173,7.484999999999999)(174,7.7295)(175,8.6785)(176,9.5195)(177,9.6065)(178,9.725)(179,9.9785)(180,10.198)(181,11.009)(182,12.105)(183,12.9335)(184,12.9895)(185,13.048)(186,13.741)(187,14.071)(188,14.6875)(189,15.607)(190,15.6495)(191,16.7285)(192,17.546)(193,19.2515)(194,19.4405)(195,20.0225)(196,20.1755)(197,21.346)(198,21.8425)(199,22.506999999999998)(200,22.9685)(201,23.0245)(202,25.990000000000002)(203,27.954500000000003)(204,28.6575)(205,28.861)(206,30.239)(207,30.689999999999998)(208,31.698)(209,33.5935)(210,33.977000000000004)(211,35.495000000000005)(212,36.542500000000004)(213,39.2845)(214,42.457)(215,43.36)(216,43.462500000000006)(217,43.7745)(218,44.855000000000004)(219,45.0345)(220,45.442)(221,45.702)(222,45.7215)(223,48.067)(224,48.7745)(225,48.899)(226,60.973)(227,62.918000000000006)(228,64.174)(229,64.305)(230,64.322)(231,65.587)(232,71.744)(233,76.832)(234,77.42349999999999)(235,78.3575)(236,81.8925)(237,83.0865)(238,85.428)(239,85.60300000000001)(240,89.4085)(241,93.1285)(242,94.14150000000001)(243,94.1545)(244,95.6335)(245,97.836)(246,101.822)(247,105.429)(248,111.1215)(249,114.4745)(250,130.3945)(251,130.39499999999998)(252,132.74099999999999)(253,133.192)(254,141.6215)(255,143.67899999999997)(256,149.081)(257,160.928)(258,167.4155)(259,172.6955)(260,173.2645)(261,178.19)(262,180.7395)(263,205.6015)(264,231.82299999999998)(265,302.8165)(266,364.9225)(267,453.5535)(268,534.2245)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,625.809)(323,628.068)(324,793.9835)(325,829.128)(326,1068.6154999999999)
        (1,0.154922)(2,0.16203)(3,0.16743999999999998)(4,0.1717455)(5,0.1776755)(6,0.18612099999999998)(7,0.192998)(8,0.2026765)(9,0.2119715)(10,0.21608899999999998)(11,0.219945)(12,0.2219755)(13,0.2316645)(14,0.235128)(15,0.2425365)(16,0.2457745)(17,0.252011)(18,0.25256850000000003)(19,0.254865)(20,0.255891)(21,0.2610625)(22,0.2653535)(23,0.2660585)(24,0.26918600000000004)(25,0.30066000000000004)(26,0.30200400000000005)(27,0.3026175)(28,0.3041345)(29,0.3067565)(30,0.30746700000000005)(31,0.31862)(32,0.32464899999999997)(33,0.3256645)(34,0.3263325)(35,0.3655485)(36,0.38409899999999997)(37,0.4118465)(38,0.425622)(39,0.430578)(40,0.43336600000000003)(41,0.448606)(42,0.45592299999999997)(43,0.483968)(44,0.4881005)(45,0.4889105)(46,0.5045935)(47,0.5082450000000001)(48,0.5188925)(49,0.5458745)(50,0.560948)(51,0.5641455)(52,0.6128235)(53,0.618761)(54,0.6312105)(55,0.6723705)(56,0.6821665)(57,0.69794)(58,0.711919)(59,0.721591)(60,0.7423455)(61,0.7961125)(62,0.7980195)(63,0.808441)(64,0.836962)(65,0.839183)(66,0.933079)(67,0.942664)(68,0.9718495)(69,0.97444)(70,0.9779344999999999)(71,0.991527)(72,0.9930885)(73,1.0209700000000002)(74,1.0946449999999999)(75,1.10531)(76,1.15149)(77,1.1866349999999999)(78,1.210845)(79,1.23458)(80,1.2388750000000002)(81,1.31433)(82,1.421795)(83,1.43323)(84,1.444695)(85,1.48672)(86,1.550775)(87,1.551265)(88,1.55156)(89,1.669785)(90,1.8561999999999999)(91,1.976875)(92,2.00042)(93,2.0389049999999997)(94,2.096415)(95,2.186255)(96,2.22913)(97,2.315905)(98,2.3898650000000004)(99,2.54013)(100,2.60611)(101,2.60944)(102,2.6443899999999996)(103,2.741485)(104,2.840595)(105,3.007345)(106,3.084695)(107,3.208935)(108,3.2174750000000003)(109,3.4957000000000003)(110,3.6079600000000003)(111,3.836605)(112,3.87767)(113,4.023855)(114,4.22523)(115,4.327075)(116,4.50767)(117,4.746745)(118,4.75872)(119,4.82061)(120,5.062799999999999)(121,5.2063950000000006)(122,5.473305)(123,5.647815)(124,5.750845)(125,5.927935)(126,5.9856)(127,6.01107)(128,6.25594)(129,6.6053999999999995)(130,6.780865)(131,7.45555)(132,7.601205)(133,8.3549)(134,8.50667)(135,8.93148)(136,9.75158)(137,9.891905)(138,10.452649999999998)(139,11.08155)(140,11.118549999999999)(141,11.83055)(142,12.226099999999999)(143,12.7446)(144,12.918099999999999)(145,13.8072)(146,14.99855)(147,15.16465)(148,15.1822)(149,15.21805)(150,15.637550000000001)(151,17.998649999999998)(152,18.0412)(153,18.66775)(154,20.0746)(155,20.2927)(156,21.0214)(157,21.14295)(158,21.7038)(159,22.141350000000003)(160,23.45805)(161,24.112450000000003)(162,25.30105)(163,26.61605)(164,26.9514)(165,28.98065)(166,30.1477)(167,32.513000000000005)(168,34.3553)(169,34.602850000000004)(170,35.5378)(171,37.0947)(172,38.03035)(173,40.04715)(174,41.0664)(175,42.72505)(176,43.044)(177,46.64125)(178,47.21875)(179,47.9634)(180,48.93729999999999)(181,49.8788)(182,51.02385)(183,51.62195)(184,52.5173)(185,53.80455)(186,54.90755)(187,55.09935)(188,55.6484)(189,61.11785)(190,64.0018)(191,67.27529999999999)(192,68.43615)(193,68.97585000000001)(194,71.16885)(195,72.803)(196,74.79355)(197,76.7559)(198,78.85485)(199,79.62270000000001)(200,84.57554999999999)(201,85.4471)(202,89.161)(203,91.00555)(204,91.6671)(205,97.90975)(206,99.47255)(207,99.60055)(208,102.1345)(209,102.7355)(210,106.424)(211,107.0495)(212,108.18)(213,111.311)(214,113.22)(215,117.193)(216,117.432)(217,118.82)(218,119.5865)(219,119.605)(220,123.08000000000001)(221,128.4465)(222,129.745)(223,130.29899999999998)(224,133.5515)(225,136.2095)(226,137.7775)(227,143.461)(228,147.75549999999998)(229,147.81400000000002)(230,150.659)(231,151.886)(232,157.6635)(233,160.24149999999997)(234,164.90050000000002)(235,169.23950000000002)(236,170.856)(237,172.566)(238,177.9085)(239,181.6165)(240,184.4385)(241,194.03199999999998)(242,196.68200000000002)(243,198.5965)(244,205.7255)(245,207.32850000000002)(246,211.034)(247,213.25900000000001)(248,214.421)(249,214.50549999999998)(250,219.112)(251,223.61700000000002)(252,225.3065)(253,227.43)(254,233.64749999999998)(255,236.6765)(256,238.001)(257,238.57150000000001)(258,243.904)(259,244.97250000000003)(260,245.851)(261,251.5865)(262,255.33)(263,256.7405)(264,256.754)(265,258.7155)(266,269.6885)(267,273.637)(268,280.01)(269,280.3825)(270,282.85900000000004)(271,294.4145)(272,299.4505)(273,307.072)(274,317.73900000000003)(275,321.061)(276,337.3365)(277,352.3805)(278,357.814)(279,367.0725)(280,381.804)(281,394.17)(282,441.2795)(283,530.3815)(284,545.6645000000001)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
\addlegendentry{ $G_1$ }

==> solver_comp_selp.tex <==
 \addplot[
    dotted,
    color=orange,
    mark=*,
    ]
    coordinates {
        (1,0.6968365000000001)(2,0.7333505)(3,0.751529)(4,0.772543)(5,0.804659)(6,0.8279460000000001)(7,0.8395475)(8,0.8681105)(9,0.8884495)(10,0.8995615)(11,0.9119785)(12,0.9463535000000001)(13,1.01375)(14,1.064155)(15,1.226655)(16,1.267335)(17,1.33013)(18,1.381665)(19,1.5247000000000002)(20,1.5453800000000002)(21,1.5910199999999999)(22,1.6478199999999998)(23,1.7503199999999999)(24,2.124355)(25,2.25526)(26,2.333435)(27,2.79624)(28,3.266605)(29,4.110595)(30,4.88972)(31,5.20197)(32,5.6643550000000005)(33,5.770004999999999)(34,5.811155)(35,6.875065)(36,7.35468)(37,7.466100000000001)(38,7.501469999999999)(39,7.518275)(40,7.752455)(41,9.400535000000001)(42,10.5714)(43,10.582705)(44,10.936)(45,12.1957)(46,12.30375)(47,14.86505)(48,17.67715)(49,19.5923)(50,22.186700000000002)(51,26.0766)(52,27.9112)(53,30.640549999999998)(54,40.0429)(55,46.2892)(56,47.8786)(57,53.77245)(58,73.4265)(59,78.30824999999999)(60,89.05015)(61,110.4155)(62,120.959)(63,141.584)(64,170.117)(65,223.565)(66,231.8475)(67,240.1805)(68,303.932)(69,350.51099999999997)(70,398.7685)(71,405.9495)(72,532.6395)(73,586.7855)(74,600.0)(75,600.0)(76,600.0)(77,600.0)(78,600.0)(79,600.0)(80,600.0)(81,600.0)(82,600.0)(83,600.0)(84,600.0)(85,600.0)(86,600.0)(87,600.0)(88,600.0)(89,600.0)(90,600.0)(91,600.0)(92,600.0)(93,600.0)(94,600.0)(95,600.0)(96,600.0)(97,600.0)(98,600.0)(99,600.0)(100,600.0)(101,600.0)(102,600.0)(103,600.0)(104,600.0)(105,600.0)(106,600.0)(107,600.0)(108,600.0)(109,600.0)(110,600.0)(111,600.0)(112,600.0)(113,600.0)(114,600.0)(115,600.0)(116,600.0)(117,600.0)(118,600.0)(119,600.0)(120,600.0)(121,600.0)(122,600.0)(123,600.0)(124,600.0)(125,600.0)(126,600.0)(127,600.0)(128,600.0)(129,600.0)(130,600.0)(131,600.0)(132,600.0)(133,600.0)(134,600.0)(135,600.0)(136,600.0)(137,600.0)(138,600.0)(139,600.0)(140,600.0)(141,600.0)(142,600.0)(143,600.0)(144,600.0)(145,600.0)(146,600.0)(147,600.0)(148,600.0)(149,600.0)(150,600.0)(151,600.0)(152,600.0)(153,600.0)(154,600.0)(155,600.0)(156,600.0)(157,600.0)(158,600.0)(159,600.0)(160,600.0)(161,600.0)(162,600.0)(163,600.0)(164,600.0)(165,600.0)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)
        };
\addlegendentry{ \texttt{selp} }

==> solver_plot_epasp.tex <==
\addplot[
    dashed,
    color=yellow,
    mark=x,
    ]
    coordinates {
    (1,0.001571)(2,0.008602499999999999)(3,0.009071)(4,0.012036999999999999)(5,0.015216)(6,0.0156585)(7,0.0156585)(8,0.0156585)(9,0.02972)(10,0.08504149999999999)(11,0.09093899999999999)(12,0.090964)(13,0.0915585)(14,0.09231600000000001)(15,0.09399550000000001)(16,0.09633749999999999)(17,0.097559)(18,0.10023)(19,0.10125)(20,0.1027975)(21,0.1073625)(22,0.10890050000000001)(23,0.1169065)(24,0.11887600000000001)(25,0.119216)(26,0.1234645)(27,0.129986)(28,0.138416)(29,0.140868)(30,0.14647949999999998)(31,0.15289799999999998)(32,0.153177)(33,0.1549975)(34,0.1613075)(35,0.18138100000000001)(36,0.182256)(37,0.185805)(38,0.1898235)(39,0.190066)(40,0.2918535)(41,0.3604)(42,0.3625795)(43,0.37163500000000005)(44,0.39266650000000003)(45,0.415846)(46,0.4331955)(47,0.503023)(48,0.5208124999999999)(49,0.659082)(50,0.668829)(51,0.6939915)(52,1.0067205000000001)(53,1.097325)(54,1.2383899999999999)(55,1.30443)(56,1.427545)(57,1.777155)(58,1.93245)(59,2.060285)(60,2.07011)(61,2.35268)(62,2.4309000000000003)(63,2.8895299999999997)(64,3.135085)(65,3.27035)(66,3.4832)(67,3.683225)(68,4.557295)(69,4.86781)(70,4.98204)(71,5.285905)(72,5.337695)(73,7.34757)(74,7.844234999999999)(75,8.480595000000001)(76,8.882615000000001)(77,10.42)(78,10.59535)(79,10.9185)(80,14.444600000000001)(81,15.455950000000001)(82,15.6878)(83,19.33175)(84,20.43385)(85,20.79965)(86,24.502299999999998)(87,24.86385)(88,25.2709)(89,27.154)(90,32.46835)(91,35.224199999999996)(92,36.6045)(93,37.29345)(94,37.52235)(95,40.977450000000005)(96,43.1949)(97,50.36805)(98,51.25925)(99,54.046400000000006)(100,55.760999999999996)(101,70.8968)(102,74.87525)(103,76.40520000000001)(104,90.53165000000001)(105,93.6799)(106,107.758)(107,120.9585)(108,157.3875)(109,197.547)(110,204.172)(111,220.253)(112,305.5425)(113,334.64099999999996)(114,352.45500000000004)(115,352.457)(116,359.1355)(117,387.92150000000004)(118,409.446)(119,412.5855)(120,440.3635)(121,474.86)(122,480.818)(123,489.6075)(124,559.0)(125,559.3405)(126,581.789)(127,591.3720000000001)(128,594.5195)(129,594.7495)(130,595.4855)(131,596.4970000000001)(132,600.0)(133,600.0)(134,600.0)(135,600.0)(136,600.0)(137,600.0)(138,600.0)(139,600.0)(140,600.0)(141,600.0)(142,600.0)(143,600.0)(144,600.0)(145,600.0)(146,600.0)(147,600.0)(148,600.0)(149,600.0)(150,600.0)(151,600.0)(152,600.0)(153,600.0)(154,600.0)(155,600.0)(156,600.0)(157,600.0)(158,600.0)(159,600.0)(160,600.0)(161,600.0)(162,600.0)(163,600.0)(164,600.0)(165,600.0)(166,600.0)(167,600.0)(168,600.0)(169,600.0)(170,600.0)(171,600.0)(172,600.0)(173,600.0)(174,600.0)(175,600.0)(176,600.0)(177,600.0)(178,600.0)(179,600.0)(180,600.0)(181,600.0)(182,600.0)(183,600.0)(184,600.0)(185,600.0)(186,600.0)(187,600.0)(188,600.0)(189,600.0)(190,600.0)(191,600.0)(192,600.0)(193,600.0)(194,600.0)(195,600.0)(196,600.0)(197,600.0)(198,600.0)(199,600.0)(200,600.0)(201,600.0)(202,600.0)(203,600.0)(204,600.0)(205,600.0)(206,600.0)(207,600.0)(208,600.0)(209,600.0)(210,600.0)(211,600.0)(212,600.0)(213,600.0)(214,600.0)(215,600.0)(216,600.0)(217,600.0)(218,600.0)(219,600.0)(220,600.0)(221,600.0)(222,600.0)(223,600.0)(224,600.0)(225,600.0)(226,600.0)(227,600.0)(228,600.0)(229,600.0)(230,600.0)(231,600.0)(232,600.0)(233,600.0)(234,600.0)(235,600.0)(236,600.0)(237,600.0)(238,600.0)(239,600.0)(240,600.0)(241,600.0)(242,600.0)(243,600.0)(244,600.0)(245,600.0)(246,600.0)(247,600.0)(248,600.0)(249,600.0)(250,600.0)(251,600.0)(252,600.0)(253,600.0)(254,600.0)(255,600.0)(256,600.0)(257,600.0)(258,600.0)(259,600.0)(260,600.0)(261,600.0)(262,600.0)(263,600.0)(264,600.0)(265,600.0)(266,600.0)(267,600.0)(268,600.0)(269,600.0)(270,600.0)(271,600.0)(272,600.0)(273,600.0)(274,600.0)(275,600.0)(276,600.0)(277,600.0)(278,600.0)(279,600.0)(280,600.0)(281,600.0)(282,600.0)(283,600.0)(284,600.0)(285,600.0)(286,600.0)(287,600.0)(288,600.0)(289,600.0)(290,600.0)(291,600.0)(292,600.0)(293,600.0)(294,600.0)(295,600.0)(296,600.0)(297,600.0)(298,600.0)(299,600.0)(300,600.0)(301,600.0)(302,600.0)(303,600.0)(304,600.0)(305,600.0)(306,600.0)(307,600.0)(308,600.0)(309,600.0)(310,600.0)(311,600.0)(312,600.0)(313,600.0)(314,600.0)(315,600.0)(316,600.0)(317,600.0)(318,600.0)(319,600.0)(320,600.0)(321,600.0)(322,600.0)(323,600.0)(324,600.0)(325,600.0)(326,600.0)(327,600.0)(328,600.0)(329,600.0)(330,600.0)(331,600.0)(332,600.0)(333,600.0)
};
\addlegendentry{\texttt{EP-ASP}}

